Private Multi-Winner Voting for Machine Learning

Private multi-winner voting is the task of revealing $k$-hot binary vectors satisfying a bounded differential privacy (DP) guarantee. This task has been understudied in machine learning literature despite its prevalence in many domains such as healthcare. We propose three new DP multi-winner mechanisms: Binary, $\tau$, and Powerset voting. Binary voting operates independently per label through composition. $\tau$ voting bounds votes optimally in their $\ell_2$ norm for tight data-independent guarantees. Powerset voting operates over the entire binary vector by viewing the possible outcomes as a power set. Our theoretical and empirical analysis shows that Binary voting can be a competitive mechanism on many tasks unless there are strong correlations between labels, in which case Powerset voting outperforms it. We use our mechanisms to enable privacy-preserving multi-label learning in the central setting by extending the canonical single-label technique: PATE. We find that our techniques outperform current state-of-the-art approaches on large, real-world healthcare data and standard multi-label benchmarks. We further enable multi-label confidential and private collaborative (CaPC) learning and show that model performance can be significantly improved in the multi-site setting.

==> contents/0abstract.tex <==
\begin{abstract}
Private multi-winner voting is the task of revealing $k$-hot binary vectors satisfying a bounded differential privacy (DP) guarantee. This task has been understudied in machine learning literature despite its prevalence in many domains such as healthcare. We propose three new DP multi-winner mechanisms: Binary, $\tau$, and Powerset voting. Binary voting operates independently per label through composition. $\tau$ voting bounds votes optimally in their $\ell_2$ norm for tight data-independent guarantees. Powerset voting operates over the entire binary vector by viewing the possible outcomes as a power set. Our theoretical and empirical analysis shows that Binary voting can be a competitive mechanism on many tasks unless there are strong correlations between labels, in which case Powerset voting outperforms it. We use our mechanisms to enable privacy-preserving multi-label learning in the \emph{central setting} by extending the canonical single-label technique: PATE. We find that our techniques outperform current state-of-the-art approaches on large, real-world healthcare data and standard multi-label benchmarks. We further enable multi-label confidential and private collaborative (CaPC) learning and show that model performance can be significantly improved in the multi-site setting.
\end{abstract}


% Private multi-winner voting is the task of revealing $k$-hot binary vectors satisfying a bounded differential privacy (DP) guarantee. This task has been understudied in machine learning literature despite its prevalence in many domains such as healthcare. We propose three new DP multi-winner mechanisms: Binary, $\tau$, and Powerset voting. Binary voting operates independently per label through composition. $\tau$ voting bounds votes optimally in their $\ell_2$ norm for tight data-independent guarantees.
% % Removed Gaussian mechanisms, this is a detail we can and do clarify later. Not needed for abstract imo.
% Powerset voting operates over the entire binary vector by viewing the possible outcomes as a power set. Our theoretical and empirical analysis shows that Binary voting can be a competitive mechanism on many tasks unless there are strong correlations between labels, in which case Powerset voting outperforms it.
% % We theoretically and empirically analyze tradeoffs showing that Powerset voting requires strong correlations between labels to outperform Binary voting.
% We use our mechanisms to enable privacy-preserving multi-label learning in the \emph{central setting} by extending the canonical single-label technique: PATE. We find that our techniques outperform current state-of-the-art approaches on large, real-world healthcare data and standard multi-label benchmarks. We further enable multi-label confidential and private collaborative (CaPC) learning and show that model performance can be significantly improved in the multi-site setting.

==> contents/31powerset_binary_comparison.tex <==
When we compare our two voting mechanisms, we find that there are two regimes where \powerset voting outperforms \binary voting. 

\emph{The first regime is when there are high correlations between the multi-winner candidates}, i.e., there is strong coordinate dependence. We find this by viewing the distribution of outcomes as a non-uniform balls and bins problem. Here, 
%(described in detail in  Section~\ref{app:binary-versus-powerset} below).
%Recall we are now operating over the power set of outcomes, i.e., each distinct multi-winner election outcome is a separate candidate and possible outcome for the single-winner election; the single-winner election has exponentially many possible outcomes in the number of multi-winner candidates $k$. 
% The distribution over outcomes can be approximated by viewing the collection of single-winner outcomes as a non-uniform balls and bins problem: 
each distinct outcome $i\in[1,\ldots,2^k]$ has some probability $P_i$ of being selected. Then, each of the $n$ ballots is an independent ball being thrown at these bins. 
%If we model each candidate of the corresponding multi-winner election as having some probability $p_j$ ($j\in [1,\ldots,k]$) then 
We can estimate the probability of each of the $2^k$ single-winner outcomes. Doing so, we find that the privacy loss may be lesser than \binary voting when the likelihood of a single $i-$th outcome is much higher than the rest---this occurs when there is high probability of $>1$ candidate outcomes occurring simultaneously. 

% if the likelihood of a single $i-$th outcome is much higher than the rest, it results in decreased privacy loss.

\emph{The second regime is when neither mechanism can leverage stronger data-dependent privacy guarantees.} When the distribution of multi-winner outcomes and single-winner outcomes approaches a uniform distribution, the best guarantee either can achieve is the data-independent privacy bound based on their sensitivity and noise variance $\sigma^2$. Because \binary voting composes $k$ separate DP queries, the privacy loss using this approach is necessarily higher than from \powerset voting which only releases a single outcome. Similar to Section~\ref{sec:sqrtk}, we find that as the distributions approach that coordinate-independence, \binary voting provides tighter analysis. See Section~\ref{app:binary-versus-powerset} for our detailed theoretical analysis and supporting empirical evidence.

% Instead, when there is coordinate independence, or when each individual candidate has a high probability of winning, or when the most likely outcomes are approximately the same between \binary voting and \powerset voting, we find that \binary voting performs better. See Section~\ref{sec:multi-pate} below for a detailed analysis of the data-independent and data-dependent privacy bounds of \binary voting and \powerset voting as well as Section~\ref{app:binary-versus-powerset} for our detailed theoretical analysis and supporting empirical evidence.

It is also possible to cast a $\tau$-multi-winner election as one $\tau$-single-winner election.
% It is also possible to incorporate $\tau$-voting into the \powerset method. A given teacher is allowed to set up to $\tau$ positive labels for a given query sample.
This limits the number of possible classes in \powerset voting from $C=2^{k}$ to $C={{k}\choose{0}} + {{k}\choose{1}} + \dots + {{k}\choose{\tau}}$ classes. This
%it increases the possibility of achieving a consensus between teachers and improves performance (faster run-time).
(1) increases the possibility of achieving a consensus
% between teachers 
% (a higher gap between max and runner-up numbers of votes can be achieved), 
(2) the data independent bound is lower (computed as: $1 - (1 / C)$), and (3) the method has faster run-time. 
%On the other hand, it does not lower the sensitivity of the Powerset mechanism because changing one of the teachers potentially decreases the vote count from one class and increase it in another one. Thus, the sensitivity remains 2. 
%Intuitively, up to $\tau$ positive labels could be selected based on the confidence of the positive value for a label, where we would choose the top $\tau$ labels with the highest confidence of being positive. However, given that most deep multi-label models use independent predictive heads (i.e., a separate sigmoid activation per output label), naively comparing these values may not lead to the best performance. Thus, no clear notion of what the desired subset is in the case that $>\tau$ candidates are present. 
\chris{likely keep just 1 graph and remove the rest.}
We present an evaluation of this approach in Appendix~\ref{sec:powerset-tau-appendix} for a real-world dataset and find that it is outperformed by the \binary voting.

% \subsubsection{Powerset with $\tau$-voting}
% \label{sec:powserset-tau}

% \amrita{Prior discussion had the three techniques separated, only this section mixes them together and I could not find any reference to this later as well, this seems a bit abrupt - maybe add 1-2 lines motivating why mixing the two techniques is needed? }\adam{We also show experiments for this method in Section 6.}
% It is also possible to incorporate $\tau$-voting into the \powerset method. A given teacher is allowed to set up to $\tau$ positive labels for a given query sample. This approach limits the number of possible classes in \powerset from $C=2^{k}$ to $C={{k}\choose{0}} + {{k}\choose{1}} + \dots + {{k}\choose{\tau}}$ classes. Since we have fewer classes: (1) it increases the possibility of achieving a consensus between teachers (a higher gap between max and runner-up numbers of votes can be achieved), (2) the data independent bound is lower (computed as: $1 - (1 / C)$), and (3) the method has higher performance (faster run-time). On the other hand, it does not lower the sensitivity of the Powerset mechanism because changing one of the teachers potentially decreases the vote count from one class and increase it in another one. Thus, the sensitivity remains 2. 

% Intuitively, up to $\tau$ positive labels could be selected based on the confidence of the positive value for a label, where we would choose the top $\tau$ labels with the highest confidence of being positive. However, given that most deep multi-label models use independent predictive heads (i.e., a separate sigmoid activation per output label), naively comparing these values may not lead to the best performance. Thus, no clear notion of what the desired subset is in the case that $>\tau$ candidates are present.

==> contents/background_backup.tex <==
\section{Background}\label{sec:background}
\subsection{Differential Privacy for Machine Learning}
\label{ssec:dp}

Differential Privacy (DP) is the canonical framework for measuring the privacy leakage of a randomized algorithm~\cite{dwork2006calibrating}. It requires the mechanism (in our work, the training algorithm), to produce statistically indistinguishable outputs on any pair of `adjacent' datasets: those differing by any but only one data point. This bounds the probability of an adversary inferring properties of the training data from the mechanism's outputs.

\begin{definition}[Differential Privacy]
\label{differential_privacy}
A randomized mechanism $\mathcal{M}$ with domain $\mathcal{D}$ and range $\mathcal{R}$ satisfies $(\varepsilon, \delta)$-differential privacy if for any subset $\mathcal{S} \subseteq \mathcal{R}$ and any adjacent datasets $X, X' \in \mathcal{D}$, i.e. $\|X - X'\|_{1} \leq 1$, the following inequality holds: $
{\rm Pr}\left[\mathcal{M}(X) \in \mathcal{S}\right] \leq e^{\varepsilon} {\rm Pr}\left[\mathcal{M}(X') \in \mathcal{S}\right] + \delta.$
% \end{equation}
\end{definition}
We use \renyi Differential Privacy (RDP)~\cite{mironov2017renyi}. Because RDP bounds the privacy loss with the \renyi-divergence, it enables tighter accounting for our mechanisms that use Gaussian noise. RDP is a generalization of 
% pure, $\delta=0$-DP 
$(\varepsilon,\delta=0)-DP$. We use standard conversions to report $(\varepsilon,\delta)-DP$.
% Our work obtains the required randomization for privacy by sampling from a Gaussian distribution. \vinith{Is it necessary to say this given we are using $\epsilon$, $\delta$ DP? +1 swapping this.} Thus, we use a generalization of DP known as \renyi Differential Privacy (RDP)~\cite{mironov2017renyi} that is well-suited to the analysis of mechanisms that involve Gaussian noise.
% RDP enables this by using the \renyi-divergence and tracking across many orders,
% generalizes pure DP (i.e., when $\delta=0$) 
% to compare the mechanism's output distributions. \vinith{Would it be better to say that RDP provides more accurate privacy accounting by using ....}

% \begin{definition}
% \textbf{R\'enyi Differential Privacy}~\cite{mironov2017renyi}. We say that a mechanism $\mathcal{M}$ is $(\lambda, \varepsilon)$-RDP with order $\lambda \in (1,\infty)$ if for all neighboring datasets $X$, $X'$:
% \[
% D_{\lambda} (\mathcal{M}(X) || \mathcal{M}(X')) = \frac{1}{\lambda-1} \log E_{\theta\sim\mathcal{M}(X')}\bigg[\bigg(\frac{p_{\mathcal{M}(X)}(\theta)}{p_{\mathcal{M}(X')}(\theta)}\bigg)^{\lambda}\bigg] \le \varepsilon
% \]
% \end{definition}
\chris{I don't think we use this much. I suggest we remove this definition.}
% \begin{definition}[Rényi Divergence]
% \label{renyi_divergence}
% For two probability distributions P and Q defined over $\mathcal{R}$, the Rényi divergence of order $\lambda > 1$ between them is defined as:
% \begin{align*}
% D_{\lambda}(P \, || \, Q) \triangleq & \frac{1}{\lambda - 1} \log\mathbb{E}_{\theta \sim Q}\left[\bigg(\frac{P(\theta)}{Q(\theta)}\bigg)^{\lambda}\right] \\ 
% =& \frac{1}{\lambda - 1} \log\mathbb{E}_{\theta \sim P} \left[ \left( \frac{P(\theta)}{Q(\theta)}\right)^{\lambda - 1}\right]
% \end{align*}
% \end{definition}

\begin{definition}[Rényi Differential Privacy]
\label{renyi_differential_privacy}
A randomized mechanism $\mathcal{M}$ is said to satisfy $\varepsilon$-Rényi differential privacy of order $\lambda$, or $(\lambda, \varepsilon)$-RDP for short, if for any adjacent datasets $X, X' \in \mathcal{D}$:
\begin{flalign*}
&D_{\lambda}(\mathcal{M}(X) \, || \, \mathcal{M}(X')) = &&\\
&= \frac{1}{\lambda - 1} \log\mathbb{E}_{\theta \sim \mathcal{M}(X)}\left[\left(\frac{{\rm Pr}[\mathcal{M}(X) = \theta]}{{\rm Pr}[\mathcal{M}(X') = \theta]}\right)^{\lambda - 1}\right] \leq \varepsilon &&
\end{flalign*},
\end{definition}
where $D_{\lambda}(P\, || \, Q)$ is the \renyi Divergence between distributions $P$ and $Q$ defined over a range $\mathcal{R}$.
It is convenient to consider RDP in its functional form as $\varepsilon_{\mathcal{M}}(\lambda)$, which is the RDP $\varepsilon$ of mechanism $\mathcal{M}$ at order $\lambda$. Our privacy analysis builds on the following result.
% We now state the result which our privacy analysis builds on.

\begin{lemma}
\label{lemma:rdp-gaussian}
\textbf{RDP-Gaussian mechanism (for a \single setting)}~\cite{mironov2017renyi}. Let $f:\mathcal{X} \rightarrow \mathcal{R}$ have bounded $\ell_2$ sensitivity for any two neighboring datasets $X, X^\prime$, i.e., $\left\lVert f(X) - f(X^\prime) \right\rVert_2 \le \Delta_2$. The Gaussian mechanism $\mathcal{M}(X) = f(X) + \mathcal{N}(0,\sigma^2)$ obeys RDP with $\varepsilon_{\mathcal{M}}(\lambda) = \frac{\lambda \Delta_2^2}{2 \sigma^2}$.
\end{lemma}

Another notable advantage of RDP over $(\varepsilon,\delta)$-DP is that it composes naturally. This will be helpful when analyzing our approach which repeatedly applies the same private mechanism to a dataset. 

% \begin{lemma}
% \label{lemma:rdp-composition}
% \textbf{RDP-Composition}~\cite{mironov2017renyi}. Let mechanism $\mathcal{M}=(\mathcal{M}_1,\dots,\mathcal{M}_t)$ where $\mathcal{M}_i$ can potentially depend on outputs of $\mathcal{M}_1,\dots,\mathcal{M}_{i-1}$. $\mathcal{M}$ obeys RDP with $\varepsilon_{\mathcal{M}}(\cdot) = \sum_{i=1}^{t}\varepsilon_{\mathcal{M}_i}(\cdot)$.
% \end{lemma}

\begin{lemma}
\label{lemma:rdp-composition}
\textbf{RDP-Composition}~\cite{mironov2017renyi}. If a mechanism $\mathcal{M}$ consists of a sequence of adaptive mechanisms $\mathcal{M}_1,\dots,\mathcal{M}_k$ such that for any $i \in [k]$, $\mathcal{M}_i$ guarantees $(\delta,\varepsilon_i)$-RDP, then $\mathcal{M}$ guarantees $(\delta,\sum_{i=1}^{k} \varepsilon_i)$-RDP.
\end{lemma}

\subsection{PATE and \capc}
\label{sec:PATE}

\textbf{PATE} (Private Aggregation of Teacher Ensembles) is a model agnostic algorithm for training ML models with DP guarantees~\cite{papernot2017semi}. Rather than training a single model on a dataset, PATE trains an ensemble of models from (disjoint) partitions of the dataset. Each model, called a teacher, is then asked to predict on a test input and to vote for one class. Teacher votes are collected into a histogram where $n_i(x)$ indicates the number of teachers who voted for class $i$. To preserve privacy, PATE relies on the noisy argmax mechanism and only reveals a noisy aggregate prediction (rather than revealing each prediction directly): ${\rm argmax}\{n_i(x) + \mathcal{N}(0, \sigma_{G}^2)\}$, where the variance  $\sigma_{G}^2$ of the Gaussian controls the privacy loss of revealing this prediction. A student model learns in a semi-supervised fashion by querying the ensemble of teachers for noisy labels, where each label incurs additional privacy loss. Loose data-independent guarantees are obtained through advanced composition~\cite{dwork2014algorithmic} and tighter data-dependent guarantees (see Appendix Section~\ref{app:data-dependent}) are possible when there is high consensus among teachers on the predicted label~\cite{papernot2018scalable}. To further reduce privacy loss, \textit{Confident GNMax} only reveals predictions that have high consensus: $\max_i\{ n_i(x)\}$ is compared against a noisy threshold also sampled from a Gaussian with variance $\sigma_T^2$. PATE was created for \single classification; our work extends it to the \multi setting. 

\textbf{\capc} (Confidential and Private Collaboration) is a distributed collaborative learning framework that extends \pate from the central to the collaborative setting~\cite{capc2021iclr}. In addition to bounding the training data DP privacy loss, \capc also protects the confidentiality of test data and teacher model parameters by introducing new cryptographic primitives. In \capc, these teacher models are known as \answeringParties and are distributed across sites, communicating via these cryptographic primitives---we use \answeringParties when referring specifically to \capc and \teacherModels otherwise.

\textit{Confidentiality} refers to the notion that no other party (or adversary) can view, in plaintext, the data of interest---it protects the inputs to our mechanism. This differs from \textit{DP} which reasons about what can be inferred from the outputs of our mechanism, in our case about the training set for each teacher model. Both protect data privacy in different ways. 
%The \capc protocol described by~\cite{capc2021iclr} is: (1) private inference of teacher models, (2) secret sharing of predictions with a Privacy Guardian who enforces DP, and (3) revealing of the DP plain-text prediction.
In \capc, each answering party is a distinct and different protocol participant with their own (teacher) model. The querying party initiates the protocol by (1) encrypting unlabeled data and the other (answering) parties return an encrypted label. Then, (2) the encrypted vote is secretly shared with both the answering party and the Privacy Guardian (PG), such that each has only one share (neither knows the label in plaintext); the PG follows PATE to achieve a $\varepsilon-DP$ bound for all the answering parties. Finally, (3) the PG engages in the secure computation with the querying party and returns an $\varepsilon-$DP vote to the querying party. The goal is to maximize both the number and quality of votes that can be returned to the querying party under a chosen $\varepsilon-$DP guarantee.
% This allows the querying party to obtain a prediction without revealing its input and without the need to centralize all of the teachers in a single location. Thus, the confidentiality of the querying party's data and of the answering parties' models is guaranteed. Through PATE, differential privacy of training data for each answering party is also guaranteed. 
The detailed CaPC protocol can be found in Algorithm~\ref{capc-protocol} of Appendix~\ref{app:capc-protocol}. 

\subsection{Prior work on \Multi Classification}
The closest to our work is that of~\cite{privateknn2020cvpr}, which provides a privacy-preserving nearest neighbors algorithm formulated using PATE. The nearest-neighbor training points are used as teachers, where their labels are the votes. Our mechanisms can similarly be used to extend this nearest-neighbour PATE formulation to the \multi setting. However, their work assumes the existence of a publicly-available embedding model (used to project the high-dimensional data to a low-dimensional manifold for meaningful nearest-neighbour distance computation). This is a strong assumption and is often not applicable to the multi-site scenario we consider.
% While this work is applicable to the \multi setting, it assumes the existence of a publicly-available embedding model, which is used to project high-dimensional data onto a sufficiently-low-dimensional manifold for the meaningful computation of distances (to determine the nearest neighbors). 
%Without this, consensus, which is required for determining the released label, would be difficult to reach. 
%\vinith{Since we frame the problem in the introduction as revealing $k$-hot binary vectors I think we should include the work on privately answering $k-way$ marginals / counting queries such as ~\cite{ganesh2020privately, dagan2020boundednoise}} 
Instead, our approach does not make this assumption. 
%and is model-agnostic, e.g., it supports deep neural networks directly. 
Further, we show in Section~\ref{sec:mainscheme} that clipping votes to the $\ell_1$ ball, as done in~\cite{privateknn2020cvpr}, is not optimal if using (the commonly used) Gaussian distribution. Instead, we obtain tighter bounds by clipping votes to an $\ell_2$ ball. 

The multi-label voting problem can also be formulated as simultaneously answering multiple counting queries which has been studied extensively in the theoretical literature. Though data-independent optimal error bounds for the privacy loss were proven by~\cite{dagan2020boundednoise}, these mechanisms do not generally have data-dependent bounds and have yet to show promise empirically in settings such as \multi voting\footnote{We explored these approaches (not shown) finding looser data-independent guarantees compared to our proposed mechanisms in our setup.}.
% optimal error bounds with probability 1 were proven using a bounded noise mechanism, deviating from the traditional Laplacian and Gaussian noise mechanisms~\cite{dagan2020boundednoise}. 
% Additionally, the Gaussian mechanism has been generalized for privately answering multiple counting queries with optimal $\ell_{\infty}$ error bounds. 
% These mechanisms have yet to show promise empirically in settings such as multi-label voting.  
Another alternative \multi method is differentially private stochastic gradient descent (DPSGD), which can be used agnostic to the label-encoding because the mechanism releases gradient updates instead of labels.~\cite{abadi2016deep} proposed and evaluated this approach in the \single setting.~\cite{AdaptiveDPSGD2021} applied it to the multi-label setting to train small \multi models ($k=5$ labels). %~\cite{AdaptiveDPSGD2021} explore the use of adaptive DPSGD to train small \multi models ($k=5$ labels) in healthcare. 
We compare directly with their work and find that our methods perform better in both small and large \multi model settings. Appendix~\ref{sec:related-work-detailed} contains a detailed description of related work.
Finally, we stress that our evaluation includes large-scale healthcare datasets with a natural need for privacy and the additional challenge of being severely imbalanced.
% , like CheXpert~\cite{irvin2019chexpert}, MIMIC-CXR~\cite{johnson2019mimiccxrjpg}, and PadChest~\cite{padchest2020}. \chris{\@ Adam can you put the two largest datasets here and use "etc." after (it pushes a new line which doesn't look good). Also, we say all the datasets multiple times so it's repeitive} 
